Incorporating Structured Representations into Pretrained Vision & Language Models Using Scene Graphs

Vision and language models (VLMs) have demonstrated remarkable zero-shot (ZS) performance in a variety of tasks. However, recent works have shown that even the best VLMs struggle to capture aspects of compositional scene understanding, such as object attributes, relations, and action states. In contrast, obtaining structured annotations, such as scene graphs (SGs), that could improve these models is time-consuming and costly, and thus cannot be used on a large scale. Here we ask whether small SG datasets can provide sufficient information for enhancing structured understanding of pretrained VLMs. We show that it is indeed possible to improve VLMs when learning from SGs by integrating components that incorporate structured information into both visual and textual representations. For the visual side, we incorporate a special "SG Component" in the image transformer trained to predict SG information, while for the textual side, we utilize SGs to generate fine-grained captions that highlight different compositional aspects of the scene. Our method improves the performance of several popular VLMs on multiple VL datasets with only a mild degradation in ZS capabilities.

==> Tables/VL-CheckList.tex <==
% \vspace{-1.0em}
\begin{table*}[t!]
    \vspace{-1.0em}
	\tablestyle{6pt}{1.}
	\scriptsize
    \centering
    \begin{small}
    \begin{tabular}{l|ccccc|cc|c}
            \toprule
             &\multicolumn{5}{c|}{Attribute} &\multicolumn{2}{c|}{Object} &\multicolumn{1}{c}{Relation}\\
             Model & Action & Color & Material & Size & State & Location & Size & Action\\
            \midrule            
            CLIP &68.1 &70.2 & 73.1 & 52.9 &63.3 &81.0 & 80.1 & 78.0 \\
            BLIP &79.5 &83.2 & 84.7 & 59.8 &68.8 &83.0 & 81.3 & 81.5\\
            BLIP2 &79.5 &83.2 & 84.7 & 59.8 &68.8 &83.0 & 81.3 & 81.5\\
            \midrule
            CLIP-SGVL (ours) &76.6 \gcol{+8.5} &78.0 \gcol{+7.8} & 80.6 \gcol{+7.5}  & 59.7  \gcol{+6.8}&61.2 \rcol{-2.1} &83.2 \gcol{+2.2} & 81.9 \gcol{+1.8} & 79.0 \gcol{+1.0} \\
            BLIP-SGVL (ours) &79.2 \rcol{-0.3} &94.5 \gcol{+11.3} & 91.9 \gcol{+7.2} & 73.3 \gcol{+13.5} &70.0 \gcol{+1.2} &86.5  \gcol{+3.5}& 83.9 \gcol{+2.6} & 81.9 \gcol{+0.4} \\
            BLIP2-SGVL (ours) &79.2 \rcol{-0.3} &94.5 \gcol{+11.3} & 91.9 \gcol{+7.2} & 73.3 \gcol{+13.5} &70.0 \gcol{+1.2} &86.5  \gcol{+3.5}& 83.9 \gcol{+2.6} & 81.9 \gcol{+0.4} \\
            \bottomrule        
    \end{tabular}
    \end{small}
    \vspace{-1.0em}
    \caption{
    \textbf{VL-Checklist Result} on the Attribute, Object, and Relation tests, excluding the Visual Genome dataset.}
    \vspace{-2.0em}
\label{tab:main_res_vlchecklist}
\end{table*}

==> Tables/Winoground.tex <==
\begin{table*}[t!]
    % \vspace{-1.0em}
    \centering
	\tablestyle{3.6pt}{1.}
	\scriptsize
    \begin{small}
    \begin{tabular}{l|ccccccccc}
            \toprule
            &\multicolumn{3}{c}{NoTag} &\multicolumn{3}{c}{Visually Difficult} &\multicolumn{3}{c}{Complex Reasoning}\\
            Model & Text & Image & group & Text & Image & Group & Text & Image & Group\\
            \midrule            
            CLIP &30.4 &11.1 & 8.2 & 15.8 & 0.0 & 0.0 & 24.4 & 7.7 & 3.8\\
            BLIP & 44.8 & 23.8 & 19.0 & 29.0 & 10.5 & 10.5 & 24.4 & 7.7 & 2.6\\
            BLIP2 & 44.8 & 23.8 & 19.0 & 29.0 & 10.5 & 10.5 & 24.4 & 7.7 & 2.6\\
            \midrule
            CLIP-SGVL (ours) &33.2 \gcol{+2.8} &14.0 \gcol{+2.9} & 8.7 \gcol{+0.5}  & 18.4 \gcol{+2.6} & 5.3 \gcol{+5.3} & 5.3 \gcol{+5.3} & 24.4  & 16.7 \gcol{+9.0} & 12.8 \gcol{+9.0}\\
            BLIP-SGVL (ours) &45.9 \gcol{+1.1} &34.3 \gcol{+10.5} & 25.6 \gcol{+6.6}  & 23.7 \rcol{-5.3} & 18.4 \gcol{+7.9} & 15.8 \gcol{+5.3} & 33.3 \gcol{+8.9} & 11.5 \gcol{+3.8} & 7.7 \gcol{+5.1}\\
            BLIP2-SGVL (ours) &45.9 \gcol{+1.1} &34.3 \gcol{+10.5} & 25.6 \gcol{+6.6}  & 23.7 \rcol{-5.3} & 18.4 \gcol{+7.9} & 15.8 \gcol{+5.3} & 33.3 \gcol{+8.9} & 11.5 \gcol{+3.8} & 7.7 \gcol{+5.1}\\
            \bottomrule        
    \end{tabular}
    \end{small}
    \vspace{-1.0em}
    \caption{
    \textbf{Winoground Results} on the NoTag, Visually Difficult and Complex Reasoning splits.}

\label{tab:res_winoground}
\end{table*}

==> Tables/ablations/Ablations-Comp.tex <==



\begin{table*}[h!]
    \centering
    \begin{small}
    \begin{tabular}{l|ccccc|cc|c}
            
            \toprule
            &\multicolumn{5}{c|}{Attribute}&\multicolumn{2}{c|}{Relation}&{21 Zero-Shot Tasks}\\
           Method & Color &	Material &	Size &	State &	 Action	& Action &	Spatial & Average\\
           \midrule
% CLIP~\cite{clip} &69.50\% &	69.70\% &	70.50\% &	61.10\% &	67.20\% &	72.10\% &	54.00\%&	\textbf{63.39\%}&	\textbf{88.82\%}\\
% CLIP + LoRA &73.15\% &	68.10\% &	68.15\% &	57.60\% &	64.41\% &	70.03\% &	41.00\% &	62.54\%	&	88.32\%	 \\
% \midrule
Ours Pos & 72.35\% &	69.25\% &	69.80\% &	59.35\% &	66.08\%& 70.97\% &	39.20\%& \textbf{55.37\%} \\
Ours RB Neg &	78.45\% &	83.20\% &	69.50\% &	\textbf{65.95\%} &	69.66\% &	75.97\% &	74.70\% &54.66\%\\
Ours LLM Neg	&	76.00\% &	79.70\% &	72.75\% &	61.35\% &	68.36\% &	77.23\% &	72.40\% &55.05\%\\
Ours RB+LLM Negs&\textbf{79.25\%} &	\textbf{84.25\%} &	72.15\% &	64.05\% &	\textbf{69.82\%} &	\textbf{79.03\%} &	\textbf{78.40\% }&54.66\%\%\\

Ours Combined&77.45\% &	77.35\% &	\textbf{73.35\%} &	62.30\% &	69.39\% &	74.70\% &	63.20\% &54.77\%\%\\

            \bottomrule
    \end{tabular}
    
    \end{small}
    \caption{\textbf{Ablation study - component analysis.} Detailed evaluation on \textit{Attribute} \& \textit{Relation} \svlc{}s.}
    \label{tab:ablation_comp_att_rel}
    \tabvspace
\end{table*}

==> Tables/ablations/ablations_old.tex <==
\begin{table*}[t]
    \vspace{-1.5em}
    % components
    % \footnotesize
    \begin{subtable}[t]{0.3\linewidth}
    \tablestyle{2.0pt}{1.0}
        \caption{{Scene Graph Information}}
        \input{Tables/ablations/abl_graph_usage}
        \label{tab:graph_usage}
     \end{subtable}
    %  \hspace
    \hfill
    \begin{subtable}[t]{0.32\linewidth}
    \tablestyle{2.0pt}{1.0}
        \caption{{Visual Encoder Components}}
        \input{Tables/ablations/abl_components}
        \label{tab:method_components}
     \end{subtable}
    %  \hspace{0.2cm}
    % \hfill
    % \begin{subtable}[t]{0.40\textwidth}
    % \tablestyle{4.0pt}{1.00}
    %     % \vspace{3cm}
    %     \centering
    %     \caption{{{\graph} Attributes}}
    %     \input{Tables/Experiments/smthelse_Relations_part}
    %     \label{tab:abl_relations}
    % \end{subtable}
    
    
    \hfill
    \begin{subtable}[t]{0.27\linewidth}
    \tablestyle{2.0pt}{1.0}
        \caption{{Image-SG Comprehensiveness}}
        \input{Tables/ablations/abl_comprehensivness}
        \label{tab:comprehensivness}
     \end{subtable}
     \vspace{-1.0em}
     \caption{\textbf{Ablations on the Winoground Dataset.} We report Text, Image, and Group scores. We show (a) The contribution of scene graph information. (b) Method components, and (c) Image-SG comprehensiveness. More ablations are in~\Secref{supp:expr} in supplementary.}
     \label{tab:ablations}
    \vspace{-1.5em}
\end{table*}

==> Tables/ablations/wrapper.tex <==
\begin{table*}[t]
    % components
    % \footnotesize
    \begin{subtable}[t]{0.1\textwidth}
    \tablestyle{0.1pt}{1.00}
        \caption{{Method components}}
        \input{Tables/Experiments/smthelse_ablation_tokens_consistency_part}
        \label{tab:abl_components}
    \end{subtable}
    %  \hspace
    \hfill
    \begin{subtable}[t]{0.18\linewidth}
    \tablestyle{6.0pt}{1.00}
        \caption{{Images Amount}}
        \input{Tables/Experiments/smthelse_data_ratio_part}
        \label{tab:abl_data_ratio}
     \end{subtable}
    %  \hspace{0.2cm}
    % \hfill
    % \begin{subtable}[t]{0.40\textwidth}
    % \tablestyle{4.0pt}{1.00}
    %     % \vspace{3cm}
    %     \centering
    %     \caption{{{\graph} Attributes}}
    %     \input{Tables/Experiments/smthelse_Relations_part}
    %     \label{tab:abl_relations}
    % \end{subtable}
    \hfill
    \begin{subtable}[t]{0.325\linewidth}
    \tablestyle{4.0pt}{1.00}
        \caption{\revision{Absence of hands/objects}}
        \input{Tables/Rebuttal/no_obj_hands_inference}
        \label{tab:no_obj_hands_inference}
     \end{subtable}
     \caption{\textbf{Ablations.} We show (a) Contributions of {\approach} components. (b) Amount of annotated images used in training. (c) Examine \revision{the robustness of {\approach} to clips that does not contain hands/contains only hands}. The experiments are performed on the SomethingElse split. For more ablations, see~\ref{supp:expr} in supplementary.}
     \label{tab:ablations}
    %  \vspace{-20pt}
\end{table*}

==> Tables/supp_all_results.tex <==
\begin{table*}[t!]
    \centering
	\tablestyle{1pt}{1.}
	\scriptsize
    \begin{small}
    \begin{tabular}{l|ccc|ccc|cc|c}
            \toprule
            &\multicolumn{3}{c|}{Winoground} & \multicolumn{3}{c|}{VL-Checklist} & \multicolumn{2}{c|}{ARO} & 
            \multicolumn{1}{c}{VSR}
            \\
            \toprule
            &\multicolumn{3}{c|}{All Dataset}
            &\multicolumn{3}{c|}{All Datasets Avg}
            & Flickr30K
            & COCO
            & All Dataset\\
            Model & Text & Image & group & Attribute & Object & Relation & Order & Order & Avg\\
            %\midrule
            %Random Chance &25.0 &25.0 & 16.7  & 50.0 & 50.0 & 50.0 & 20.0 & 20.0 & 50.0 & -\\ 

            % \midrule 
            % % LXMERT~\cite{tan2019lxmert} &27.5 &8.7 & 6.0  & 71.4 & 82.4 & 69.4 & - & - & -& -\\
            % % $\text{UNITER}_{base}$~\cite{Chen2020UNITERUI} &32.2 &13.2 & 10.0  & 68.0 & 81.9 & 75.3 & - & - & -& -\\
            % % ViLT (ViT-B/32)~\cite{vilt} &34.7 &14.0 & 9.2  & 72.2 & 86.3 & 75.6 & - & - & -& -\\ 
            % CLIP (ViT-B/32)~\cite{radford2021learning} &30.7 &10.5 & 8.0  & 65.5 & 80.6 & 78.0 & 59.5 & 46 & - & 56.4\\
            % NegCLIP(ViT-B/32)~\cite{Yuksekgonul2022WhenAW} &29.5 & 10.5 & 8.0  &  &  & & 91.0  & 86.0  & - & \\
            % % CLIP MT~\cite{radford2021learning} &30.75\% &10.5\% & 8\% & 30.41\% & 11.11\% & 8.19\% & 30.41\% & 11.11\% & 8.19\% & 0\%\\
            % BLIP (ViT-B/16)~\cite{blip} &39.0 &19.2 & 15.0 & 75.2 & 82.2 & 81.5 & 27.9 & 24.9 & 56.5 &  49.0\\
            % BLIP2~\cite{blip} &39.0 &19.2 & 15.0 & 75.2 & 82.2 & 81.5 & 27.9 & 24.9 & 56.5 &  49.0\\
            % % BLIP MT~\cite{blip} &39\% &19.25\% & 15\% & 44.77\% & 23.84\% & 19 & 30.41\% & 11.11\% & 8.19\% & 0\%\\
            \midrule
            FLAVA  & 32.3 &20.0 & 14.5  & 54.6 & 70.6 & 46.6 & 12.9 & 3.9 & 54.1\\
            ViLT  &34.8  &14.0 &9.3   &73.3  &85.0  &62.0  &22.4  &18.7  & -\\
            \midrule 
            % LXMERT~\cite{tan2019lxmert} &27.5 &8.7 & 6.0  & 71.4 & 82.4 & 69.4 & - & - & -& -\\
            % $\text{UNITER}_{base}$~\cite{Chen2020UNITERUI} &32.2 &13.2 & 10.0  & 68.0 & 81.9 & 75.3 & - & - & -& -\\
            % ViLT (ViT-B/32)~\cite{vilt} &34.7 &14.0 & 9.2  & 72.2 & 86.3 & 75.6 & - & - & -& -\\ 
            CLIP  & 30.7 &10.5 & 8.0  & 65.5 & 80.6 & 78.0 & 59.5 & 46.0 & -\\
            % CLIP MT~\cite{radford2021learning} &30.75\% &10.5\% & 8\% & 30.41\% & 11.11\% & 8.19\% & 30.41\% & 11.11\% & 8.19\% & 0\%\\
            BLIP  &39.0 &19.2 & 15.0 & 75.2 & 82.2 & 81.5 & 27.9 & 24.9 & 56.5\\
            BLIP2 &42.0 &23.8 &19.0  &77.8  &84.9  &84.9  &33.9 &32.3 & 61.9\\
            % BLIP MT~\cite{blip} &39\% &19.25\% & 15\% & 44.77\% & 23.84\% & 19 & 30.41\% & 11.11\% & 8.19\% & 0\%\\
            \midrule 
            NegCLIP & 29.5 & 10.5 & 8.0  &68.0  &81.4  & 81.3 & 91.0  & 86.0  & - \\
            NegBLIP  &42.5 &24.0 &18.5  &78.2  &83.7  &81.9  & 85.0  & 84.7  & 57.9 \\
            NegBLIP2 & 41.5 & 26.0 & 20.5  & 79.0  &87.0  &88.2  &91.8   & 88.2 & 62.1  \\
            \midrule
            CLIP-SGVL (ours) &32.0 \gcol{+1.3} &14.0 \gcol{+3.5} & 9.8 \gcol{+1.8}  & 72.0 \gcol{+6.5} & 82.6 \gcol{+2.0} & 82.0 \gcol{+4.0} & 82.0 \gcol{+22.5} & 78.2 \gcol{+32.2} & -\\
            BLIP-SGVL (ours) &42.8 \gcol{+3.8} &27.3 \gcol{+8.1} & 21.5 \gcol{+6.5} & 81.8 \gcol{+6.6} & 85.2 \gcol{+3.0} & 81.9 \gcol{+0.4} & 70.0 \gcol{+42.1 } & 71.0 \gcol{+46.1} & 62.4 \gcol{+5.9}\\
            BLIP2-SGVL (ours) &42.8 \gcol{+0.8} &28.5 \gcol{+4.5} &23.3 \gcol{+4.3}  & 81.2 \gcol{+3.4}  &88.4 \gcol{+3.5}  &88.8 \gcol{+3.9}  &77.0 \gcol{+43.1}  &77.0 \gcol{+44.7}  & 63.4 \gcol{+1.5}\\
            \bottomrule        
    \end{tabular}
    \end{small}
    % \vspace{-1.0em}
    \caption{
    \textbf{Winoground, VL-Checklist, ARO and VSR Results}. The \green{gains} and \red{losses} are relative to the pretrained base models. We do not report CLIP-based models and ViLT on VSR since the task requires assigning a true or false label to an image-text pair. CLIP and ViLT, however, does not allow this to be done in a straightforward manner.}
    % \vspace{-1.5em}
    \label{supp:tab:res_main}
\end{table*}

==> Tables/vsr_aro.tex <==
\begin{table*}[t!]
    % \vspace{-1.0em}
    \centering
	\tablestyle{2.7pt}{1.}
	\scriptsize
    \begin{small}
    \begin{tabular}{l|cc|cccccccc}
            \toprule
            &\multicolumn{2}{c|}{ARO-PRC} & \multicolumn{8}{c}{VSR}\\
            \toprule
            Model & COCO & Flickr30K & Adjacency & Directional & Orientation & Projective & Proximity & Topological & Unallocated & Average\\
            \midrule 
            Random Chance & 20 & 20 &50 &50 &50 &50 &50 &50 &50 & 50 \\
            \midrule
            CLIP &46.0 &59.5 & - & - & - & - & - & - & - & -\\
            NegCLIP &86.0 &91.0 & - & - & - & - & - & - & - & -\\
            BLIP  & 24.9 & 27.9 & 55.4 & 48.9 & 53.7 & 58.2 & 56.5 & 55.6 & 63.4 & 56.5\\
            \midrule
            CLIP-SGVL (ours) & 87.2 \gcol{+41.2} & 91.0 \gcol{+31.5} &- & - & -& -& -& - & -  & -\\
            BLIP-SGVL (ours) &67.0 \gcol{+42.1} & 67.6 \gcol{+39.7} & 57.7 \gcol{+2.3} & 54.1 \gcol{+5.2} & 57.8 \gcol{+4.1} & 63.8 \gcol{+5.6}& 57.8 \gcol{+1.3}& 64.8 \gcol{+8.8} & 68.8 \gcol{+5.4} & 62.4 \gcol{+5.9}\\
            \bottomrule        
    \end{tabular}
    \end{small}
    \vspace{-1.0em}
    \caption{
    \textbf{Results on ARO and VSR.} We report accuracy on the ARO dataset~\cite{yuksekgonul2023when} and VSR~\cite{Liu2022VisualSR} datasets.}

\label{supp:tab:res_aro_vsr}
\end{table*}
